Ironing the Graphs: Toward a Correct Geometric Analysis of Large-Scale Graphs

Graph embedding approaches attempt to project graphs into geometric entities, i.e, manifolds. The idea is that the geometric properties of the projected manifolds are helpful in the inference of graph properties. However, if the choice of the embedding manifold is incorrectly performed, it can lead to incorrect geometric inference. In this paper, we argue that the classical embedding techniques cannot lead to correct geometric interpretation as they miss the curvature at each point, of manifold. We advocate that for doing correct geometric interpretation the embedding of graph should be done over regular constant curvature manifolds. To this end, we present an embedding approach, the discrete Ricci flow graph embedding (dRfge) based on the discrete Ricci flow that adapts the distance between nodes in a graph so that the graph can be embedded onto a constant curvature manifold that is homogeneous and isotropic, i.e., all directions are equivalent and distances comparable, resulting in correct geometric interpretations. A major contribution of this paper is that for the first time, we prove the convergence of discrete Ricci flow to a constant curvature and stable distance metrics over the edges. A drawback of using the discrete Ricci flow is the high computational complexity that prevented its usage in large-scale graph analysis. Another contribution of this paper is a new algorithmic solution that makes it feasible to calculate the Ricci flow for graphs of up to 50k nodes, and beyond. The intuitions behind the discrete Ricci flow make it possible to obtain new insights into the structure of large-scale graphs. We demonstrate this through a case study on analyzing the internet connectivity structure between countries at the BGP level.

==> bak/intro.bak.tex <==

\section{Introduction}
Graphs have emerged as fundamental conceptual tools in a large set of scientific domains. The strong point of graphs is that they capture very complex interactions into a relatively simple framework. This explains the wide usage of graphs in a wide spectrum of settings. Nevertheless, graphs exhibit very complex structures that make them difficult to analyse. Graph embedding approaches have become a major tools to simplify graphs' analysis. These techniques project the graph into a manifold defined over a metric space. The manifold should capture the fundamental properties of the underlying phenomenon represented by the graph, while simplifying the extraction of non-trivial information from it and the analysis. However, choosing the relevant manifold among the infinity of possible manifolds is challenging. Moreover, by definition the graph is  discrete, and the projection to a richer analogic continuous space will bring additional and difficult to filter artefacts that might not come from the fundamental nature of the graph, but rather results from the specific choice of manifolds. In this context, it is important to develop constructive graph embedding techniques that are backed by strong theoretical and fundamental basis and avoid introducing spurious artefacts. This is the goal of this paper. 

We will base our approach on the discrete Ricci flow applied on the Ollivier-Ricci (OR) curvature defined on graphs. This approach is motivated by the application of the continuous Ricci flow, introduced in \cite{Hamilton88}, to the proof of the Poincar{\'e} conjecture on 3-manifolds by Perelman\cite{Perelman2003}. Intuitively, the Ricci flow acts on the surface of a manifold by deforming the distances proportionally to its Ricci curvature, such that the manifold translate into a constant curvature surface. In other terms, the Ricci flow plays the role of a steam iron that is pressing over the complex manifold wrinkles and makes it similar to a flat sheet by distorting the geodesic distance over the manifold. Recently, Ollivier extended the differential geometric concept of Ricci curvature, initially defined on differentiable manifolds, to graphs that are discrete in nature \cite{OLLIVIER2007}. This extension uses optimal transport as a proxy to transpose to discrete context the classical definition of Ricci curvature that is dependent on the differentiability of the manifold. A recent paper have shown the deep connections between the OR curvature and the Ricci curvature of an embedding manifold \cite{OllivierRicciConvergence2021} by proving that the OR curvature calculated over a random geometric graph, {\em i.e.}, a graph obtained by choosing random point over a manifold and connecting points that are at distance less than a threshold $\epsilon$, converge to the Ricci curvature of the manifold when the density of random point is large enough and the threshold $\epsilon$ converges toward 0. This result opens the way for a new type of graph embedding that follows a fundamental geometric and analytic property that is at the core of the Poincar{\'e}-Perelman Theorem: the convergence of the Ricci flow.  The fact that this embedding is based on a strong mathematical basis make it more robust and strengthen the application that use the graph embedding, like graph clustering. This is the main theoretical motivation of the results presented in this paper.

Differently from isometric embeddings that try to embed a given graph into a manifold while trying to reduce as much as possible the distance distortion (the difference between edge weights in the initial graph and the distance in the projected manifold), the Ricci Flow embedding we present in this paper distort the distance between nodes in the graph in order to obtain the embedding of the modified graph into a trivial constant curvature manifold. In other terms, differently from classical embedding technique that aims into finding a complex manifold capturing the structure of the graph, the discrete Ricci flow applied to OR curvature of a graph acts like an ironing of the graph that flatten the embedding manifold and condense structural information of the graph into a set of distance or weights defined over each link of the graph. The distances are distorted in such a way that links that act as bottlenecks are stretched, while links that are in a densely connected region are compressed. 

While the application of the discrete Ricci flow to the OR curvature has already been proposed in the literature, in particular to do clustering \cite{Sia2019OllivierRicci,Ni2019Community}, this is only through more recent papers that all the theoretical components of embedding resulting from discrete Ricci flow to the OR curvature have been assembled. One major contribution of this paper, in our view, is that it connect a disparate set of research work into a theoretically strong comprehensive process resulting into
the embedding of a given graph into a simple manifold with constant curvature but condensing structural information into weights on the graph links. For this purpose we have to make a journey from the differential geometry of Riemannian manifold, to optimal transport defined over a graph and the resulting OR curvature for graphs, to applying a deforming Ricci flow that will provide the embedding of the  a given graph into a simple manifold with constant curvature but with graph edge weights that are condensing structural information. We will dedicate the section \ref{sec:theo} to the description of this journey. 

The derivation of the optimal transport and the OR curvature over each link of the graph is at the core of the approach we will follow. While, as will be described later, this optimal transport is an instance of linear programming that is known to have a polynomial complexity for most practical settings, calculating curvature over a link entails obtained a distance matrix between all neighbours of both extremity of the link. Obtaining this matrix is the most time costly elements of the calculation that are the core of the embedding we propose. While, calculating  shortest path distance between two graph nodes is $\mathcal{O}(n)$,  deriving tenths of millions of shortest paths, as is needed for practical large scale graph, can become soon intractable. A second contribution of this paper is to propose algorithmic shortcuts to enable fast calculation of the distance matrices that are at the core of the OR curvature derivation. Describing how to derive the curvatures leveraging parallel multi-thread implementation is the topic of section \ref{sec:algo}.

The main outcome of the Ricci flow embedding is the derivation for each link of a distance  that is related to the structural properties. These distances are useful for a large set of purposes. Clustering is an application that has been already reported \cite{Ni2019Community}. Nonetheless, application of such clustering has been limited because of the high complexity of deriving the OR curvature. The algorithmic implementation, described in section \ref{sec:algo}, can help to overcome these clustering complexity challenge. We will describe in section \ref{sec:appli} the use of the Ricci flow distances to evaluate the robustness and the connectivity between countries in the global Internet, opening new applications for such embeddings.








==> intro_old.tex <==
\section{Introduction}

\textcolor{purple}{Graphs have become a fundamental tool in a wide range of scientific domains, capturing complex interactions through a relatively simple framework of node-to-node relations. Yet, understanding the structure and global properties of a graph remains a daunting task, as a significant number of graph-related questions fall into the category of NP-hard problems. The history of mathematics demonstrates that frequently, the most elegant and intuitive method of simplifying complex problems is reinterpreting them as geometric problems. At the heart of geometry, there is the study of sizes, shapes, positions, angles, and dimensions of space. Geometric properties result from the interaction of the intrinsic features of geometrical objects with the extrinsic properties of the space in which they are embedded. In classical geometry, the underlying space is assumed to be homogeneous, so the local geometry of space at all points is the same. Examples of such "simple" spaces include Euclidean, spherical, and hyperbolic spaces, each defined through variations of the fifth Euclid postulate relative to the possibility and number of parallel lines passing through any point. In classical geometry, geometric properties are only related to shapes and are not affected by deformations in the underlying space. Differential geometry expands classical geometry by developing tools to account for the distortion of shapes induced by the space.
Conducting a geometric analysis of graphs involves identifying a suitable space in which the graph can be projected and studied in terms of the resulting embedding properties. A geometric analysis of the graph must incorporate the characteristics of the underlying space at every point, effectively replicating the approach devised in differential geometry. The objective of this paper is to envision how to construct a geometric analysis of graphs that is easy to interpret and can be leveraged to analyze the inherent mechanisms captured by the graph. Specifically, the goal of our study is to study how to generate faithful embeddings that are interpretable and useful for experts studying graphs.\\
\textbf{The Curvature:} In Riemannian geometry, the curvature is a measure of how much a geometric object deviates from being flat. The curvature of space serves to differentiate and comprehend the properties of any space in relationship with Euclidean space. In particular, the Ricci curvature measures how much the volume of a small ball around that point deviates from the volume of a small ball around a point on a flat surface and aggregates that deviation for a point. Recently, Ollivier extended the differential geometry concept of Ricci curvature, initially defined on differentiable manifolds, to discrete objects \cite{OLLIVIER2007}, by defining the "{\em Ollivier-Ricci curvature}" (ORC). This extension is based on a characterization of curvature in terms of optimal transport, a mathematical framework that finds the most efficient way to move mass from one probability distribution to another while minimizing the distance traveled. A recent paper has shown the equivalence between the OR curvature and the Ricci curvature of an embedding manifold \cite{OllivierRicciConvergence2021} by proving that the ORC calculated over a random geometric graph, {\em i.e.}, a graph obtained by choosing random point over a manifold and connecting points that are at a distance less than a threshold $\epsilon$, converge to the Ricci curvature of the manifold when the density of random point is large enough and the threshold $\epsilon$ converges toward 0. This result opens the way for a new type of graph embedding that follows a fundamental geometric and analytic property at the core of the Poincar{\'e}-Perelman Theorem: the convergence of the Ricci flow on manifolds. The approach in this paper is to leverage these theoretical properties to propose a framework for the geometric analysis of graphs. \\ 
\textbf{Ricci Flow:} Our approach projects the graph into a constant curvature manifold through a "{\em discrete Ricci flow}" applied on the "{\em Ollivier-Ricci curvature}" (ORC) as computed on the graph. This approach is motivated by the use of the "continuous Ricci flow", introduced in \cite{Hamilton88}, into the proof of the Poincar{\'e} conjecture on 3-manifolds by Perelman~\cite{Perelman2003}. Intuitively, the Ricci flow acts on the surface of a manifold by deforming the distances proportionally to its Ricci curvature, such that the manifold is converted to a constant curvature surface. In more intuitive terms, the Ricci flow plays the role of a smoothing steam iron that is pressing over the wrinkles or the folds of the complex initial manifold, {\em i.e.}, distorting the distances over the manifold, and transforming it into a flat sheet. Differently from classical isometric embedding techniques for graphs that recover a complex manifold by minimizing the distance distortion, {\em i.e.}, the difference between edge weights in the initial graph and the distance in the projected manifold, the discrete Ricci flow applied to OR curvature of a graph flattens the embedding manifold, into a constant curvature one, and condense structural information of the graph into a set of distance or weights defined over each link of the graph. The distances are distorted in such a way that links that act as bottlenecks are stretched, while links that are in a densely connected region are condensed. This provides precisely the type of embedding we have described above to retrieve distances This embedding strategy draws a parallel with a well-known strategy that builds on a strong mathematical backbone. In particular, the Ricci flow provides an off-the-shelf technique to smooth-out noisy structures while preserving meaningful topological information. While proving that the properties from the continuous Ricci flow can be transposed to the discrete version we describe here is still an open question, we believe this relationship is sufficient motivation to pursue this direction. Finally, we illustrate through our results that the two properties appear to be conserved in the discrete scenario. \\
\textbf{Prior Efforts:} There have already been several attempts to provide geometric interpretations of graphs. For example, graph embedding techniques \cite{Cai2018} map nodes, or edges into a low dimensional vector defined over a Euclidean space. However, for most graph embedding methods the relevant projection space is a Riemannian manifold, and the relevant distance metric is not the Euclidean distance between points but the geodesic distance calculated over this manifold~\cite{ROBLESKELLY20071042}. While traditional embedding approaches have found a large set of applications, {\em e.g.}, graph clustering \cite{LUO20032213}, links prediction and graph alignment \cite{doi:10.1073/pnas.0305199101}, graph robustness and resilience \cite{10.5555/979922.979965}, classification tasks in machine learning\cite{4359350}, {\em etc.}, they are unsatisfactory from a geometric perspective. \textbf{Pas sur que ce soit une raison suffisante pour justifier qu'ils ne soient pas bon. Il faut expliquer en quoi ca ne fait pas l'affaire pour certaines taches.} Large-scale graphs often cannot be embedded in a single geometric space \cite{}. Distances calculated over the different out-links vertex cannot be compared, as the underlying space might be different over different geodesics, {\em e.g.}, in a cylindrical space the distances in the direction going along the cylinder and the direction turning around the cylinder, have not the same interpretation. More importantly, distances cannot be interpreted beyond a single hop neighborhood, since essential metric properties like triangular inequality might not be globally valid as the distances over different hops might be emanated from different geometric spaces.}

Graphs have emerged as fundamental conceptual tools in a large set of scientific domains as it can capture very complex interactions into the relatively simple framework of node to node relation. Nevertheless, a graph is still a complex artifact and understanding its structure and global properties is a daunting task as a large set of questions relative to graphs falls in NP-hard problems. The history of mathematics evolution has shown that frequently the most elegant and intuitive way of simplifying complex problems has been to re-interpret into the framework of geometry, one of the oldest branches of mathematics. It is therefore interesting to investigate if graphs are amenable to a geometric analysis. This paper is mainly motivated by this question. 

Geometry studies the sizes, shapes, positions, angles, and dimensions of things that deploys in space. The interplay between the extrinsic properties of the underlying space and the intrinsic features of the  geometrical object create geometric properties. In classical geometry, it is assumed that the underlying (or embedding) space is such that the local geometry of space at all points is the same, {\em i.e}, the space looks the same at every point and in every direction. Example of such "simple" spaces are the Euclidean, spherical and hyperbolic spaces that are each defined through variation of the fifth Euclid postulate relative to the possibility and the number of parallel lines coming through any point. Therefore in classical geometry, geometric properties are only related to shapes and not to variations in the underlying space. Differential geometry expand classical geometry by developing tools to account for the properties of the underlying space in the properties of shapes, making possible to analyse geometric properties of shapes on differentiable manifold where the properties of shapes interplay with the variable properties, at different points, of the underlying space.
%The beauty of classical geometry resides in the fact that with a very limited set of global space properties, {\em e.g.}, the five Euclid postulates for Euclidean spaces, one can characterize a whole set of geometric and topological properties for objects lying on this space.
Developing a geometric analysis for graphs consist of finding a relevant space where graphs can be projected and where they can be studied in terms of geometric properties, {\em i.e.}, sizes, shapes, positions, angles and dimensions. However, if the embedding space is not a simple space, the geometric analysis of the graph should integrate the characteristics of the underlying space at each point, {\em e.g.}, distance might not have the same interpretation in different directions. The goal of this paper is to develop a geometric analysis of graphs that will be easy to interpret, {\em i.e.}, the impact of the embedding space can be alleviated, and that is useful for understanding to the underlying interaction process the graph is representing.
%While geometric elements like points, lines, triangles, {\em etc.}, are by nature discrete, their dimensions that are studied through geometry are of continuous nature, and therefore geometry is one of the first area in mathematics that have bridged the gap between discrete and continuous spaces. Geometry leverages the fundamental properties of the underlying space to find non-intuitive properties, like the three medians of a triangle meet a the centroid that divides each median in the ratio 2:1. 


Recently, Ollivier extended the differential geometry concept of Ricci curvature, initially defined on differentiable manifolds, to graphs that are discrete in nature \cite{OLLIVIER2007}, by defining the "{\em Ollivier-Ricci curvature}" (ORC). This extension uses optimal transport as a proxy to transpose to discrete context the classical definition of Ricci curvature that is dependent on the differentiability of the manifold. A recent paper have shown the deep connections between the OR curvature and the Ricci curvature of an embedding manifold \cite{OllivierRicciConvergence2021} by proving that the ORC  calculated over a random geometric graph, {\em i.e.}, a graph obtained by choosing random point over a manifold and connecting points that are at distance less than a threshold $\epsilon$, converge to the Ricci curvature of the manifold when the density of random point is large enough and the threshold $\epsilon$ converges toward 0. This result opens the way for a new type of graph embedding that follows a fundamental geometric and analytic property that is at the core of the Poincar{\'e}-Perelman Theorem: the convergence of the Ricci flow on manifold. The approach in this paper is to leverage on these theoretical properties to propose a framework for geometric analysis of graphs.

We will base our approach on projecting (embedding) the graph into a constant curvature manifold through a "{\em discrete Ricci flow}" applied on the "{\em Ollivier-Ricci curvature}" (ORC) defined on graphs. The Ricci flow defines a distance metric over links that can be used to develop a geometric analysis of the graph. This approach is motivated by the use of the "continuous Ricci flow", introduced in \cite{Hamilton88}, into the proof of the Poincar{\'e} conjecture on 3-manifolds by Perelman~\cite{Perelman2003}. Intuitively, the Ricci flow acts on the surface of a manifold by deforming the distances proportionally to its Ricci curvature, such that the manifold transforms into a constant curvature surface.  In more intuitive terms, the Ricci flow plays the role of a smoothing steam iron that is pressing over the wrinkles or the folds of the complex initial manifold, {\em i.e.}, distorting the distances over the manifold, and transform it into a flat sheet. 


 Differently from classical isometric embedding technique that aims into finding a complex manifold capturing the structure of the graph by minimizing the distance distortion, {\em i.e.}, the difference between edge weights in the initial graph and the distance in the projected manifold, the discrete Ricci flow applied to OR curvature of a graph acts like an ironing of the graph that flatten the embedding manifold, into a trivial constant curvature one, and condense structural information of the graph into a set of distance or weights defined over each link of the graph. The distances are distorted in such a way that links that act as bottlenecks are stretched, while links that are in a densely connected region are compressed. This  provides precisely the type of embedding we have described above to retrieve distances The fact that this embedding is based on a strong mathematical basis make it more robust and strengthen the application that use the graph embedding, like graph clustering. This is the main theoretical motivation of the results presented in this paper.

There have been already several attempts into providing geometric interpretations of graphs. For example, graph embedding techniques \cite{Cai2018} maps nodes, or edges into a low dimensional vector defined over an Euclidean space. However, for most of graph embedding methods the relevant projection space, where the projected points are lying, is a complex Riemannian manifold, and the relevant distance metric is not the Euclidean distance between points but rather a geodesic distance calculated over this complex manifold~\cite{ROBLESKELLY20071042}. While classical embedding approach have found a large set of applications, {\em e.g.}, graph clustering \cite{LUO20032213}, links prediction and graph alignment \cite{doi:10.1073/pnas.0305199101}, graph robustness and resilience \cite{10.5555/979922.979965}, classification tasks in machine learning\cite{4359350}, {\em etc.}, they are unsatisfactory from a geometric perspective. The complexity of the manifold embedding the graph is such that it cannot be described by a single geometric space. This entails that distances calculated over the different out-links vertex cannot be compared, as at the underlying space might be different over different geodesics, {\em e.g.}, in a cylindrical space the distance in the direction going along the cylinder and the direction turning around the cylinder have not the same interpretation. Moreover distances cannot be interpreted beyond a single hop neighborhood as global properties like triangular inequality might not be valid as the distances over different hops might be derived over different geometric spaces.

%In differential geometry terms, the atlas of the embedding manifold contains several charts that depends on the individual graph. That is making impossible to extract geometric properties relevant to the all parts of the graphs, {\em e.g.,} distances cannot be rescaled to be compared in different part of the graph.  
Conversely to the classical graph embedding techniques, the approach presented in this paper results in the embedding of the graph in a constant curvature manifold that is known through the Killing-Hopf theorem \cite{nla.cat-vn2569772} to be isometric to a single geometric space, the quotient of a sphere, Euclidean space, or hyperbolic space . In these spaces geometric interpretation is simpler as all direction and all point in the space are equivalent, and this is only the shapes and the distances that characterize the geometric properties. Moreover, distance resulting from our proposed embedding can be added to go beyond the single hop neighborhood as all nodes of the graphs will be projected to the same simple geometric space and geometric inequality will be valid for them. 

In addition to describing the graph projection to a constant curvature space, this paper will also show three case studies for the geometric analysis of graphs: robust spanning trees over road maps, the structural analysis of AS level connectivity graphs extracted from BGP feeds, and DO WE NEED A THIRD CASE. The first two case analyse the connectivity (through roads or BGP connections) between different geographical regions and countries and analyse if we can detect virtual obstacles in the connectivity that can be related to real geographical artefact, like oceans to cross, or political and geopolitical restrictions. This two example position this  paper as the dual of \cite{10.1145/3547353.3522645}, where delay information coming from large scales trace-routes between RIPE-ATLAS anchors are used to extract the network connectivity graph of large clouds providers. In this paper, we suppose we have the graph, and we retrieve the expected hardship of moving from one point to another, that is measured by the delay in \cite{10.1145/3547353.3522645}.


%Let's use an analogy to get a better grasp of the problem we are tackling in this paper. Let's suppose we are looking at a classical geographical road's map, and we observe that a road connects city A to B. Indeed the Euclidean distance, {i.e}, the distance as crow  flies, is not very relevant in such map, as the road might cross a mountain, a narrow bridge or a frontier that will increase the preference of  alternative paths that might go through other cities. Road's maps use the type of road,  \em{e.g.}, highway, or mountain road, and the topography, \em{i.e.}, an indication of the height, to help the viewer to choose the best paths among all possible one.  One can therefore extract from a road map a graph where two nodes, {\em i.e.}, cities or geographic points, are connected  when a direct road between them exists, and weight the link by a metric, separate from the Euclidean distance, that is relevant to the geographical and topographical properties of the environment of the road, {\em e.g.}, in terms of travel time. A relevant concept in geography is the isochronous anamorphic maps \cite{Stępień_Tomasz_The_2016} where a distance deformation calculated using the point to point metrics is used to generate a distorted geographic map, where the Euclidean distances are directly proportional to the point to point metrics. Now let's assume one has only access to the unweighted graph representing the connectivity between geographic locations over a road's map, can we retrieve the metric and through it the geographic, geometric and topological properties of the environment of the road, like presence of mountains or bottlenecks. This paper's ambition is precisely to deal with this inference problem.

%Formally speaking, a road's map represents a three dimensions manifold along with an embedded road's graph. Indeed, general graph are not embedded in 3D geography, and we need to extend the approach to general graph embedding. Graph embedding has become a major tools to simplify the structural analysis of graphs. These techniques project the graph into a manifold, {\em i.e.}, a multidimensional surface  defined over a metric space, that captures the fundamental properties of the underlying phenomenon represented by the graph. The structural properties of the graph are thereafter extracted from this manifold through geometric approaches that simplifies the extraction of non-trivial information. Choosing, for a given graph, a relevant embedding manifold, among the infinity of possible ones, needs to introduce some additional constraints. In this paper, we will consider trivial embedding manifolds with constant curvature, {\em i.e.} plane, sphere or hyperboloid, where the structural information is not anymore in the topography but fully condensed in the distances between points. In other terms, large distance in the embedding manifold will mean the presence of "virtual mountains, frontiers or bottlenecks", similar to real geographical artefact in road's map, while short one will induce easy access between two points. For such embeddings, characterizing the full manifold is irrelevant, as it does not capture structural information, and we need only need to infer the distance metrics. This is a simpler, but still challenging problem.

%While this problem seems to be motivated by geography and road maps, it has a large set of applications, {\em e.g.}, graph clustering \cite{LUO20032213}, links prediction and graph alignment \cite{doi:10.1073/pnas.0305199101}, graph robustness and resilience \cite{10.5555/979922.979965}, classification tasks in machine learning\cite{4359350}, {\em etc.}



%Moreover, by definition the graph is  discrete, and the projection to a richer analogic continuous space will bring additional and difficult to filter artefacts that might not come from the fundamental nature of the graph, but rather results from the specific choice of manifolds. In this context, it is important to develop constructive graph embedding techniques that are backed by strong theoretical and fundamental basis and avoid introducing spurious artefacts. This is the goal of this paper.

The methods we will describe in this paper is involving several mathematical tools and entails a journey from the differential geometry of Riemannian manifold, to optimal transport defined over a graph and the resulting OR curvature for graphs, to applying a deforming Ricci flow that will provide the embedding of the  a given graph into a simple manifold with constant curvature but with graph edge weights that are condensing structural information. We will dedicate the section \ref{sec:theo} to the description of this journey. 

The derivation of the optimal transport and the OR curvature over each graph's link is the central element of the methods in this paper. Calculating the OR curvature entails solving an optimal transport problem that is an instance of linear programming,  well-known to have a polynomial complexity for most practical settings. However, this linear programming instance get as input a distance matrix between all neighbours of both extremity of any edge of the graph. Deriving this matrix is the most time costly elements of the calculation, as it involves finding tenths of millions of shortest path distances in the graph for practical large scale graphs. Indeed, calculating  shortest path distances has a linear complexity $\mathcal{O}(n)$. But  deriving tenths of millions of shortest paths, can become soon intractable. A contribution of this paper is to propose algorithmic shortcuts to enable fast calculation of the distance matrices in a multithreaded environment. The description of this implementation is the topic of section \ref{sec:algo}. This will extend the applicability of graph clustering techniques using discrete Ricci flow \cite{Sia2019OllivierRicci,Ni2019Community} that has been limited  because of the high complexity of deriving the OR curvature, to more realistic applicative settings involving graphs with tenths of thousands of nodes.

In the  section \ref{sec:appli}, we will validate the method and describe the use of the Ricci flow distances to evaluate the robustness and the connectivity between countries in the global Internet.  

